SAMPLE-HD: Simultaneous Action and Motion Planning Learning Environment

Humans exhibit incredibly high levels of multi-modal understanding - combining visual cues with read, or heard knowledge comes easy to us and allows for very accurate interaction with the surrounding environment. Various simulation environments focus on providing data for tasks related to scene understanding, question answering, space exploration, visual navigation. In this work, we are providing a solution to encompass both, visual and behavioural aspects of simulation in a new environment for learning interactive reasoning in manipulation setup. SAMPLE-HD environment allows to generate various scenes composed of small household objects, to procedurally generate language instructions for manipulation, and to generate ground truth paths serving as training data.

==> Sections/baseline.tex <==
\section{Baseline model}

The task of predicting the steering can be realised with the use of various inputs. In the baseline approach we draw inspiration from symbolic approaches to visual reasoning and present a method that facilitates the importance of using the visual feedback.

%  \begin{figure*}[t]
%      \centering
%      \includegraphics[width=0.85\linewidth]{Images/nips_model.pdf}
%      \caption{Diagram of the suggested baseline approach. Note colour coding corresponding to various stages of the method - red is the flow of visual information through Mask R-CNN and attributes extraction providing scene representation, blue represents translation of the instruction to symbolic program via seq2seq network, purple corresponds to program execution, and green relates to controller and exchange of the information with the environment.}\label{fig:model}
%  \end{figure*}

Our model, similarly to NS-VQA and SHOP-VRB, consists of several stages, namely, program predictor, scene segmentation, attributes extraction, program execution, robot controller. The diagram of the approach is presented in Figure \ref{fig:model}. All models are trained with single Nvidia RTX 2080Ti GPU. For the training we randomly split dataset into training and test data with $7912$ tasks for the former and $448$ for the latter (corresponding to respectively $1900$ and $100$ scenes). 
% \red{image somewhere here}

\paragraph*{Program prediction} We use attention sequence-to-sequence \cite{Sutskever2014SequenceNetworks} translation model with bidirectional LSTM encoder and LSTM decoder. The encoder hidden state is used to initialise decoder which predicts a set of program tokens. A sequence of symbolic programs are constructed in a way that when executed on disentangled scene representation, it provides a compact, precise task description - including type, subject, and target.

\paragraph*{Program execution} Program executor follows the pattern introduced in CLEVR-IEP \cite{Johnson2017InferringReasoning}. However, we remove the assumptions on the uniqueness of the objects in the resulting answer. The output from program executor consists of 3 values - type of the task (see Table \ref{tab:instructions}), subject of the task as the list of pointers to scene objects, and the target of the task as either table part or specific object (\eg stacking task).

\paragraph*{Segmentation} The images are segmented using Mask R-CNN \cite{He2017MaskR-CNN} implemented as a part of Detectron2 \cite{Wu2019Detectron2} project.

\paragraph*{Attributes extraction} The masked images of every object are used to trained attributes extractor based on ResNet-50 network \cite{He2016DeepRecognition}. We classify every image into separate properties using classification heads (trained with cross-entropy) for each of the properties (\eg name, colour). We also predict a size and position of the objects with regression head trained to minimise mean absolute error. Given that we construct a list of properties for every object in the scene providing its disentangled representation.

\paragraph*{Controller} For the baseline experiment we have chosen a simple controller working in semi-open loop. We have decided to use robot joint coordinates in the feedback loop. Based on those at every step we calculate the expected position of the end effector of the manipulator. In the first frame provided by the environment, a pipeline of predicting the task and estimating the disentangled scene representation is executed. Based on the estimated positions of the objects in the scene, a sequence of positions for the effector is composed. For the grasping of each object we follow a simple procedure of moving above the object, approaching the grasp (with some offset if the object size is estimated to be larger that gripper fingers span), closing the gripper and following with the movement to the target position where the object is released. When destination is specified as a part of the table, target position is estimated to be far from another objects on that table part and table part boundaries.

\subsection{Experiments}

We perform baseline experiments with the use of the aforementioned method. We train Mask R-CNN for $60000$ iterations with $4$ images per batch and learning rate of $0.02$ for the SGD optimiser. Both program prediction and attributes extraction are trained with Adam \cite{Kingma2015Adam:Optimization} with learning rate of $0.001$, program prediction with batch of $256$ for $1000$ iterations, attributes extraction with batch of $24$ for $100000$ iteration. For segmentation we use loss as described in \cite{He2017MaskR-CNN}. Program tokens and categorical properties are trained with cross-entropy, while regressed values minismise L1 distance.

\paragraph*{Results} We test our approach on $448$ test instructions using different number of stages in the proposed pipeline substituting the rest with ground truth values. The results are presented as following:
\begin{itemize}
    \item Ground truth tasks + ground truth attributes - $38.6\%$
    \item Predicted tasks + ground truth attributes - $38.6\%$
    \item Predicted tasks + attributes predicted given ground truth segmentation - $11.8\%$
    \item Predicted tasks + attributes predicted from predicted segmentation - $11.6\%$
\end{itemize}
For all experiments in $3$ trials the error remained within the range of different results for $2$ tasks ($0.4\%$).

We can observe the challenging nature of the task. Simple controller without explicit visual feedback is not capable of perfectly solving the task. Grasp estimation based on the rough size of the target object is not sufficient to achieve high grasping accuracy emphasising the importance of SAMPLE-HD providing precise physics calculation with high quality visual feedback. Additionally, visual feedback facilitates better capability of collision avoidance. Further, we may note a significant drop in the performance when providing estimated parameters of the scene to the system. Potential reasons may include: inaccurate segmentation, incorrect scene description, either for categorical values or estimated positions. We have observed very high accuracy of segmentation and categorical attributes estimation - models tested with ground truth and predicted masks achieved $>98\%$ accuracy. Mean squared error of position prediction was within the range of $2cm$. Seemingly small error was noted to be the reason of the increased number of failures - even a small displacement can easily cause grasping procedure failure. This further highlights the importance of visual feedback that allows for quick position corrections.

% \begin{itemize}
%     \item Max acc simple controller: $38.6\%$ (173, 448)
%     \item : $11.8\%$ (53, 448)
%     \item : $11.6\%$ (52, 448)
% \end{itemize}

% \red{Maybe what tasks failed the most?}

% \begin{itemize}
%     \item point out importance of position prediction - mb cite categorical accuracy and mse/mae - point that small changes may break a lot
% \end{itemize}


==> Sections/related_work.tex <==
\section{Related work}


\paragraph*{Visual reasoning} Our work is closely related to visual reasoning task where the task is formulated in form of an instruction/question directly related to the visual scene. There is a large variety of datasets related to the task of visual reasoning. The first group consists of real image data and with manual annotations - VQA 2.0 \cite{Goyal2017}, GQA \cite{Hudson2019GQA:Visualreasoning.net}, VizWiz \cite{Gurari2018VizWizPeople} and various extensions for different tasks (NLVR2 \cite{Suhr2019APhotographs}, VCR \cite{Zellers2019FromReasoning}) or detailed scene annotations (Visual Genome \cite{Krishna2017VisualAnnotations}). The second group consists of synthetic datasets with procedurally generated images. The main representative of the group is CLEVR \cite{Johnson2017CLEVR:Reasoning} and related works \cite{Liu2019CLEVR-Ref+:Expressions, Johnson2017InferringReasoning, Santoro2017AReasoning}. Further works build upon scene generation by providing new objects in the scenes - Minecraft scenes in \cite{Yi2018Neural-SymbolicUnderstanding} or realistic home appliances in SHOP-VRB \cite{Nazarczuk2020SHOP-VRB:Perception}. Other methods focus on new challenges in different tasks - ACRE \cite{Zhang2021ACRE:Covariation}, TRANCE \cite{Hong2021TransformationReasoning}, V2A \cite{Nazarczuk2020V2A-VisionLanguage}.

Several approaches were proposed to perform visual reasoning, in particular end-to-end methods (MAC \cite{Hudson2019CompostionalReasoning},  FiLM \cite{Perez2018FiLM:Layer}), including various schemes for fusing multi-modal data from text and image: LXMERT \cite{Tan2019LXMERT:Transformers}, ViLT  \cite{Kim2021ViLT:Supervision}, ViLBERT \cite{Lu2019ViLBERT:Tasks, Lu202012-in-1:Learning}, bottom-up \cite{Anderson, Jiang2020InAnswering}. A different category of methods is related to reasoning over the graphs. Basic graph reasoning was introduced with RN \cite{Santoro2017AReasoning}, and BCN \cite{Chang2018BroadcastingReasoning}, followed by methods utilising graph neural networks - LCGN \cite{Hu2019Language-ConditionedReasoning}, \cite{Teney2017Graph-StructuredAnswering}, MGN \cite{Saqur2020MultimodalAnswering}. Finally, visual reasoning was approached with modular methods, either via stacking neural network modules (NMN \cite{Andreas2016NeuralNetworks}), or by predicting symbolic programs to be executed on the disentagled scene representation - initialised by CLEVR-IEP \cite{Johnson2017InferringReasoning}, followed with NS-VQA \cite{Yi2018Neural-SymbolicUnderstanding}, NS-CL \cite{Mao2019TheSupervision}.
In our work, we propose a baseline method for action planning that is based on the symbolic approach.

\paragraph*{Navigation in 3D environments}
A number of simulated environments were introduced along with the task of visual navigation in 3D space and  realistically looking indoor synthetic scenes were proposed  such as Matterport3D \cite{Chang2017Matterport3D:Environments}, House3D \cite{Wu2018BuildingEnvironment}, Room2Room \cite{Anderson2018Vision-and-LanguageEnvironments}, and Habitat \cite{Savva2019Habitat:Research}. Embodied Question Answering \cite{Das2018EmbodiedAnswering, Yu2019Multi-TargetAnswering} was introduced as a combination of visual reasoning and navigation. VLN \cite{Huang2019TransferableNavigation} also explored navigation based on both vision and language.

\paragraph*{Interaction in 3D environments} 
Important area of related work is focused on various interactions with objects, often including navigation. DeepMind Control Suite \cite{Tassa2018DeepMindSuite} addresses various control tasks for different robotic agents. Surreal \cite{Fan2018SURREAL:Benchmark} is a reinforcement learning framework for manipulation tasks. RoboTurk \cite{Mandlekar2019ScalingDexterity} introduces a rich base of crowd-sourced demonstrations for different tasks to provide a base for imitation learning. AI2THOR \cite{Kolve2017AI2-THOR:AI} and RoboTHOR \cite{Deitke2020RoboTHOR:Result} provide a simulated navigation environment that enables primitive interactions with  objects.
ALFRED \cite{Shridhar2020ALFREDTasks} adopts the aforementioned simulator in order to set a benchmark for understanding language instructions in robotics. In \cite{Nagarajan2020LearningEnvironments} the focus is  on exploration for learning object affordances. Grasping of home objects is explored in \cite{Gupta2018RobotBias}. Imitation learning for manipulators is investigated in \cite{Xie2020DeepManipulation}, whereas \cite{Stepputtis2020Language-ConditionedTasks} expands the task through language conditioning. ManipulaTHOR \cite{Ehsani2021ManipulaTHOR:Manipulation} provides an object manipulation functionality within AI2THOR considering grasping as a discrete action (\ie object is gripped when \textit{pick} command is executed in its proximity). SAPIEN \cite{Xiang2020SAPIEN:ENvironment} is a simulator focusing on the articulations between objects' parts. IKEA Furniture Assembly \cite{Lee2021IKEATasks} provides a benchmark for various assembly tasks.

In this work we propose a simulated environment for  manipulation of small objects with robotic arm equipped with a gripper.  In contrast to existing environments e.g. operating on discrete interactions with object (\ie one action \textit{pick} immediately changes the state of the object to \textit{picked}) our simulator offers scenes of a high visual quality and precise simulation of interactions.




% \begin{itemize}
%     \item mention action space, usually discrete - e.g. RoboThor - set of fixed turns makes it a different task - also discrete angles may not work for manipulation
%     \item Go for scene understanding - VQ, Visual Reasoning, referring expressions, object discovery, set prediction
%     \item Embodied task - how they developed 
%     \item exploration (Learning Affordance Landscapes for Interaction Exploration in 3D Environments)
%     \item affordance learning?
%     \item robotics - manipulation, steering prediction (usually cars but still related), grasp prediction
%     \item simulated environments - mostly RoboThor, Ai2Thor
% \end{itemize}
